PRRS Outbreak Prediction via Deep Switching Auto-Regressive Factorization Modeling

We propose an epidemic analysis framework for the outbreak prediction in the livestock industry, focusing on the study of the most costly and viral infectious disease in the swine industry -- the PRRS virus. Using this framework, we can predict the PRRS outbreak in all farms of a swine production system by capturing the spatio-temporal dynamics of infection transmission based on the intra-farm pig-level virus transmission dynamics, and inter-farm pig shipment network. We simulate a PRRS infection epidemic based on the shipment network and the SEIR epidemic model using the statistics extracted from real data provided by the swine industry. We develop a hierarchical factorized deep generative model that approximates high dimensional data by a product between time-dependent weights and spatially dependent low dimensional factors to perform per farm time series prediction. The prediction results demonstrate the ability of the model in forecasting the virus spread progression with average error of NRMSE = 2.5\%.

==> tex/extra.tex <==











\section{Dynamic Mode Decomposition}
\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\linewidth]{ICCASP2022/fig/graph.pdf}
\caption{Graph state snapshots in time. The state measurements $x_n$ represent .}
\label{fig:graph}
\end{figure}
\label{sec:dmd}
In this section, we describe how we can use DMD to model and analyze infection disease data. The primary goals of computational epidemiology is to investigate how a livestock population interacts with a virus in the context of a plethora of complex phenomena.
The key concept in modeling the data was to abstract the population
into groups according to their disease status. For example, people that are susceptible to acquiring a disease are grouped into a state called S. The population that is currently infected with the disease is grouped into the state I and the recovered in R.

In this section we talk about DMD, a powerful data-driven method to extract spatial temporal coherent structures from high dimensional data and give you a linear model for how those evolve in time. 
\subsection{Infectious Disease Data}
DMD can analyze snapshots of infectious disease data from experiments, numerical simulations, or historical records to extract coherent spatio-temporal patterns. Data collected from separate spatial locations can be formed into vectors representing state snapshots that evolve in time. In fluid dynamics, the measured state $x_k$ is clearly related to the physics, for example, the velocity, vorticity, and stream functions at each discretized spatial grid point. For well-curated disease data, as found in the output of detailed numerical simulations, the choice of states $x_k$ may be equally well defined, for example, the number of infections in a given spatial node. For data collected from the field, an aggregation step is required across both space and time. Often the data arrives in the form of individual patient records with a time and location stamp. To form the data matrices, the records have to be binned in space and time. Temporally resolving the individual records depends on the time scales involved in disease transmission. One natural choice for units of time is the average duration of an incubation for the disease. In space, politically defined boundaries such as states, counties, or cities are often used. After deciding on the aggregation, each pair of state snapshots $x_k$ and $x_{k+1}$ can be collected and formed into the DMD data matrices: 
\begin{equation}
{\small
\boldsymbol{X}=\begin{bmatrix}
| & | &  & |\\
\x_1 & \x_2 &\dots &\x_{N-1}\\
| & | &  & |
\end{bmatrix},~ 
\boldsymbol{X}'=\begin{bmatrix}
| & | &  & |\\
\x_2 & \x_3 &\dots &\x_N\\
| & | &  & |
\end{bmatrix}}
\end{equation}

where each column represents a different snapshot in time. Each row describes a specific state of the system, see figure.~\ref{fig:graph}.




\subsection{DMD}
I organize this data into these big matrices X and X prime okay so the columns of X the X matrix are essentially the columns of my data reshaped into sorry my snapshots of data reshaped into very very tall column vectors that are evolving in time so x1 is a big column vector where I take my my flow field at time one and I reach a pit into a tall column vector X 2 is the next snapshot X 3 is the next snapshot and so on and so forth so the columns are essentially evolving in time along with the dynamics of this system.  I'm collecting data from either a simulation or an experiment and I'm stacking.

$X'$  is that exact same data matrix but advanced one time step into the future okay so instead of X at time one at time two at time three X prime is shifted 1 delta T in the future so it's X at time 2 X at time 3 X at time 4 and so on and so forth. 

\par what the dynamic mode decomposition does is it essentially tries to find a best fit linear operator a that advances X into X prime. [Peter Schmidt's paper is basically try to find the best fit linear operator a that best agrees with this data the best maps X into X prime]
you definitely don't want to actually compute this a matrix let alone look at things like its eigenvalues and eigenvectors okay so what the DMD actually does is it approximates the leading eigen decomposition of the leading eigenvalues and eigenvectors of this a matrix without ever actually computing the a matrix.

\textbf{once you get those leading eigen values and eigen vectors of a essentially you can interpret any eigenvector of a has the shape of one of these column vectors and that i ghen vector of a can be reshaped into a flow field so these are kind of eigen flow fields that are these dominant spatial parent modes and the nice thing is because their eigenvalues they correspond to a coherent time dynamics either pure tone sine and cosine waves or pure exponential decay or exponential growth or combinations kind of growing or decaying sines and cosines so getting the leading dominant eigen decomposition of this a matrix gives you these spatial temporal coherent modes these these dominant coherent structures and it also gives you the I gain values the time dynamics of how these modes evolve in time} and so if I had kind of this leading eigen decomposition of a I could use that to predict how my system will evolve in the future by essentially predicting those future dynamics and recombining these modes to figure out what my state will do in the future okay so DM D is extremely useful it can be used for Diagnostics you can just use these modes to understand more about the physics and the flow structures and kind of what's driving your system of interest you can also use DMD to get an actual model this kind of the eigenvalues of a give you a model for how these these modes evolve in time and eventually we're gonna see that you can use these linear models for things like control okay so that's kind of where we're going okay good now here's the actual guts of what goes on under the hood to compute DMD because remember I don't want to compute that gigantic you know million by million a matrix so instead what I do in most fluid systems and in most high dimensional complex dynamical systems of interest disease modeling neuroscience fluids if you collect enough snapshots of data in time what you usually find is that there are dominant coherent patterns that emerge okay so even if there's a million degrees of freedom of your system in this case of vortex shedding there's a pre repeatable low dimensional set of patterns that emerge from those dynamics so the first step in DMD is essentially computing a singular value decomposition of this big data matrix X to find your dominant coherent structures which the columns of this you matrix so for those of you who are familiar with the proper orthogonal decomposition this is just the PIO D and these columns of U are your p OD modes and they're organized hierarchically from most important to least important in terms of capturing the variance of X ok so in many systems even if I have a million by thousand matrix I might be able to approximate it with the first five columns or first ten columns of this U matrix so this will be the first five or ten PID modes ok so then what we do is instead of writing X prime equals a times X we substitute in the singular value decomposition here so it's now a times the singular value decomposition of X and I could compute what the big a is by taking the pseudo inverse so one of the nice things about singular value decomposition is it's easy to invert this v-star because it's nor it's a unitary matrix so I multiply on the right by V then I multiply on the right by Sigma inverse and then I multiply on the right by you complex conjugate transpose and I can in pseudo inverse all of this stuff to isolate what a is okay but we don't actually want to compute the million by million a and so instead what we do is we project a onto these dominant singular vectors U star and U and we get this smaller a tilde so if I had a thousand snapshots in time this would be a thousand by thousand matrix instead of a million by million matrix okay and so then I can actually isolate this a tilde directly from the data that I have okay so I take the SVD of X so I have u Sigma and V I have X Prime and I compute this quantity here which is this little a tilde matrix and the way I think about a tilde a tilde is a linear best-fit dynamical system that tells me how my p OD modes evolve in time how these these dominant coherent patterns evolve in time okay and so this is a much much smaller matrix it's maybe thousand by thousand one hundred by hundred and it has the same use as the big a matrix okay so that's something you can prove you can actually go through this formulation and prove that this little a tilde has the same eigen values the same nonzero eigen values as big a and so I can compute the eigen decomposition of this little matrix to figure out what my eigen values of the big matrix are okay so that's the step here I do a tilde W equals W lambda so W are my eigen vectors and lambda are my eigen values of my reduced dynamic operator a tilde okay and so now I have the eigen values but what I really wanted were the eigen vectors of a I wanted these because those eigen vectors are these mode shapes over here those are my dominant coherent structures and so the last step to so I have the eigen vectors of my little projected a matrix and now the last step is to get these these big eigenvectors of the original a matrix using this formula here and this is actually the formula from Jonathan twos 2014 jcd paper this is slightly different than the original formulation that that Peter Schmidt wrote down and it Jonathan two actually proved that these high dimensional eigen vectors are actual eigenvectors of the original a matrix but basically you can just compute these you know what all of these matrices are these are your little eigenvectors of a tilde these are the matrices from your singular value decomposition and this is your big time shifted data matrix and so you can compute all of these you can get the eigen values and the the eigen vectors of the big a matrix without ever actually computing the big a matrix you're only working on this little a tilde matrix okay so that's actually the entire d-md algorithm it's really like four or five lines of code in MATLAB to do this entire procedure it's super simple if you have X and X Prime you can do all of this and it's very very fast and scalable to get these these eigenvalues and eigenvectors okay something else I'll point out that's not in this simple formulation is this is the exact SVD so if this was a million by thousand matrix I would have a thousand modes here and I would get a thousand by thousand a mate a tilde and a thousand eigenvalues and a thousand eigenvectors but if my system has really really low dimensional behavior like I can describe X with the first five columns of U and capture let's say 99\% of the energy of the system then I can substitute all of these by the first five columns of U the first five by five block of Sigma and the first five columns of V and then what I get out is this reduced SVD and I get a little 5x5 a tilde this is even more reduced it's just the dynamics on those first five p OD coefficients and then I get five DMD eigenvalues in five DMD modes okay we call these eigenvectors modes because they're spacial temporal coherent mode shapes okay so that's all there is that's how you actually compute DMD you essentially this is what DMD is defined as is essentially the leading eigenvalues and eigenvectors of that big a matrix but you compute them without ever actually resorting to building this gigantic million by million a matrix okay and once you have that you can actually get future state predictions so now that you have your modes and your eigen values if you know what your amplitudes of each of those modes are this is kind of your initial condition of how how much each of those modes is expressed in your data then you can run this forward in time you can essentially take these eigenvalues to the higher and higher powers or e to the lambda T and predict what your system will do in the future okay so that actually works pretty well for periodic systems like this so if you have a high dimensional system that has some dominant periodic or quasi periodic behavior you can actually get a really good approximation even if it's strongly non-linear with this very simple linear DMD now if you have strong transients or intermittent phenomena or non stationary behavior then it gets more complicated and you have to resort to kind of fancier regressions and a more general nonlinear framework okay what I really want to emphasize though is that all the DMD is and this is something Jonathan to pointed out all the DMD is is a best fit linear model for measurements X into one time step in the future X Prime it's a best fit linear model and so essentially you can use all of the powerful techniques of regression to find this DMD model so for example I could I could do different types of regression noise robust regression or sparsity promoting regression to find other variants of this this a matrix okay and so that's kind of the big picture overview of what DMD is it's a procedure where you take your data you stack it into matrices and you find the eigenvalues and eigenvectors of a hypothetical best fit linear operator so i took this picture from from my wife bing and this is kind of a cute representation just pictorially of what the dmt is so we did this first step of the singular value decomposition to do a dimensionality reduction step that's basically the principal components that's what the principal components analysis does is it takes high dimensional data and minds it for the fewest the fewest dominant patterns that explain that data and then DMD is essentially what you would get if principal components and the Fourier transform in time had a baby okay so you basically build this linear regression model on principal components or p OD modes or SVD modes they're all the same thing you build this linear regression model a tilde this little model that tells me how the principal components evolve and then I diagonalize that linear model to find what are the dominant patterns in time what are the type of frequencies of how linear combinations of these principal components evolve in time okay so DM D is this adorable kind of mashup of principal components in space and the Fourier transform in time okay okay one last thing a shameless plug we did write a book on this the dynamic mode decomposition this is a cyan book Nathan cuts myself being Brunton and Josh Proctor and so if you're interested in DMD if you want to know about the extensions and applications if you want to go through code you can read all about it here and work it out for yourself okay so basically that's the dynamic mode decomposition in a nutshell there's a lot more under the hood there's tons of extensions of this for what if I didn't have full state measurements what if I didn't have measurements that were resolved in time what if I'm actively trying to control my system what if I have noise


\subsection{DMD for Infectious Disease Data}
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{ICCASP2022/fig/DMD.png}
\caption{DMD.}
\label{fig:graph}
\end{figure}





\subsection{ASFV Outbreak Simulation Data}
\subsection{The Epidemiological Interpretation of DMD Modes}

